Is Big Data Performance Reproducible in Modern Cloud Networks?

Performance variability has been acknowledged as a problem for over a decade by cloud practitioners and performance engineers. Yet, our survey of top systems conferences reveals that the research community regularly disregards variability when running experiments in the cloud. Focusing on networks, we assess the impact of variability on cloud-based big-data workloads by gathering traces from mainstream commercial clouds and private research clouds. Our data collection consists of millions of datapoints gathered while transferring over 9 petabytes of data. We characterize the network variability present in our data and show that, even though commercial cloud providers implement mechanisms for quality-of-service enforcement, variability still occurs, and is even exacerbated by such mechanisms and service provider policies. We show how big-data workloads suffer from significant slowdowns and lack predictability and replicability, even when state-of-the-art experimentation techniques are used. We provide guidelines for practitioners to reduce the volatility of big data performance, making experiments more repeatable.

==> bw_emulation.tex <==

\section{Cloud Network Emulator}\label{sec:exp_setup}\label{sec:emulator}

To assess the impact of network variability on big data applications, we emulate the variability conditions described in Section~\ref{sec:netw_var}. \emph{In our context, emulation entails running real-world applications, on real-world hardware, to which we induce network bandwidth variability, as observed in Section~\ref{sec:netw_var}}. We believe this type of experimentation is superior to the other two alternatives: (i) simulation, or (ii) directly running applications on clouds. For the former, we believe the behavior of big data applications under network performance variability is far too subtle and complex to properly simulate while modeling and capturing all possible variables.

For the latter, we perform the emulation in an isolated setup, i.e., a private cluster, that does not share resources. This allows us to test in isolation the effects of network performance variability, excluding as much as possible all other sources of variability one could encounter in a cloud (e.g., CPU, memory bandwidth, I/O etc.). If we were to directly run applications in a cloud, it would have been difficult to separate the effects of network variability from, for example, the effects of CPU variability. Moreover, under emulation, network behavior is directly under our control, as opposed to the possible dynamically changing behavior of clouds.

We introduce an emulation framework for assessing the impact of network bandwidth variability on big data processing workloads. We empirically show that our framework is able to model the token-bucket variability scenario presented in Section~\ref{sec:netw_var}. %: (i) the A-H gigabit setups presented in Figure~\ref{fig:bw_distribution}, and (ii) the post-gigabit behavior found in  \amazon{}. 
We exclusively focus on the token-bucket behavior of \amazon{} and leave the \google{} behavior for future work, as well as the extremely noisy variability of \surf{}.
More in-depth investigation into the specific virtual network stacks is needed so that a high-quality emulation could be achieved.
\todo[inline]{Please Check! Is this good enough?}
%from this study, as our preliminary results show that this kind of variability is not too impactful for big data applications. We leave for future work an investigation of how such networks could impact HPC-like applications, which are more sensitive to networking.
%\todo[inline]{add something stronger here}

We implement the network emulation framework~\cite{our_traces} using as low-level traffic shaping mechanisms a combination of the Linux \emph{tc} tool, and \emph{wondershaper}~\cite{wondershaper}. A network emulation daemon runs on each cluster compute node, and listens for commands from an emulation coordination manager. The manager ensures that all nodes emulate similar network behaviors by imposing an emulation \emph{policy}. %Table~\ref{tab:emulation_policies} summarizes the policies we emulate.

\iffalse 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{Bandwidth variability emulation policies.}
\vspace*{-0.2cm}
\resizebox{0.98\columnwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
               & \textbf{Bandwidth}    & \textbf{Policies}          & \textbf{Variability}                   \\ \midrule
Ballani~\cite{ballani2011towards} & gigabit      & A-H, Figure~\ref{fig:bw_distribution}      & every X seconds \\
\amazon{}            & post-gigabit & token bucket      & app. dependent \\
%\google{}         & post-gigabit & traffic policing & app. dependent     \\
%\surf{}      & post-gigabit & N/A               & every X seconds                           
\bottomrule
\end{tabular}
}
\label{tab:emulation_policies}
\vspace*{-0.4cm}
\end{table}
\fi  


\iffalse
\subsection{Experimental Workflow}

The \yel[Visual needed]{logical workflow} of our experiments is as follows. We use 12 physical machines in our private cluster. We limit the VMs network bandwidth according to each of the eight bandwidth distributions depicted in Section~\ref{sec:netw_var}. For each bandwidth setup, we a subset of the HiBench suite~\cite{huang2010hibench}, and a subset of the TPC-DS~\cite{tpcds} suite. Each application is executed at least 10 times.
The big data workloads are run on top of Apache Spark~\cite{zaharia2010spark}, the de-facto big data analytics processing engine.

\subsection{Hardware and Software Platforms}

We perform our experiments on the local private DAS-5 cluster~\cite{bal2016medium}. Each compute node is equipped with a dual-eight-core Intel Haswell E5-2630-v3 CPUs and 64GB memory. The nodes are connected by FDR InfiniBand providing a theoretical peak bandwidth of 54Gb/s.

The compute nodes run Spark 2.4.0, Hadoop 2.7.3, and HiBench, and TPC-DS versions... The OS is Linux 3.x.x, 
\fi

\textbf{Static Bandwidth Emulation.} We first assess whether our emulation framework is able to sustain static bandwidth distributions, at lower values than what the physical links of our infrastructure could handle. We use the \emph{iperf3}~\cite{tirumala2006iperf} tool to measure the achieved performance. We set pairs of servers to communicate using two different bandwidth values, that are subsequently used for emulating the \amazon{} token bucket. Figure~\ref{fig:bw_limit_v2} shows the achieved bandwidth when limited to $bw \in \{1, 10\}$ Gb/s. We notice that the achieved values are, in practice, slightly lower than the theoretical limitation. This is expected and it is important to notice that the difference is minimal (i.e., below 1\%).

\begin{figure}[t]
\vspace*{-1cm}
\centering
\subfigure {
		\includegraphics[width=0.45\linewidth]{images/1000mbps.pdf}	
}
\subfigure{
		\includegraphics[width=0.45\linewidth]{images/10000mbps.pdf}	
}

\vspace*{-1.8cm}
\caption{Emulation of non-variable bandwidth distributions: $bw = 1Gbps$ (left), and $bw = 10Gbps$ (right).}
\label{fig:bw_limit_v2}
\vspace*{-0.3cm}
\end{figure}
% \begin{figure}[tp]
% \centering
% \subfigure[Bandwidth target = 1,000 Mbit/s \label{fig:bw_limit1000_v2}] {
% 		\includegraphics[width=0.47\linewidth]{bw_limit/1000mbps.eps}	
% }
% \subfigure[Bandwidth target = 10,000 Mbit/s \label{fig:bw_limit10000_v2}]{
% 		\includegraphics[width=0.47\linewidth]{bw_limit/10000mbps.eps}	
% }
% \vspace{-0.4cm}
% \caption{Emulation of two non-variable bandwidth distributions, when $bw \in \{1Gbps, 10Gbps\}$.}
% \label{fig:bw_limit_v2}
% \vspace*{-0.4cm}
% \end{figure}

\iffalse
\textbf{Gigabit-Era Bandwidth Emulation.} We ensure that the network bandwidth emulator is able to model the A-H distributions presented in Figure~\ref{fig:bw_distribution}. Without loss of generality, in this work, we only consider scenarios where the achievable bandwidth of one VM changes during the course of a single experiment as per the A-H distributions every few seconds. Figure~\ref{fig:emul_cloudA_gigabit} plots expected and achieved bandwidth when emulating cloud bandwidth distribution B from Figure~\ref{fig:bw_distribution}. In this experiment, the bandwidth of the servers performing the experiment varies every 5 seconds. 

\begin{figure}[]
    \centering
    \includegraphics[width=0.75\columnwidth]{images/emul_Ballani_A.pdf}
    \vspace*{-0.4cm}
    \caption{Emulation of cloud network bandwidth distribution A from Figure~\ref{fig:bw_distribution}, when the performance changes every 5 seconds. The similar aspect of the two curves indicates that emulation is high-quality.}
    \label{fig:emul_cloudA_gigabit}
    \vspace*{-0.5cm}
\end{figure}
\fi 

\textbf{Amazon Token-Bucket Bandwidth Emulation.} We ensure that the network bandwidth emulator is able to model the token-bucket mechanism and policy employed by the \amazon{}. Figure~\ref{fig:aws_emulation_validation} plots the real-world behavior encountered in the \amazon{} in comparison with our emulation. This experiment is a zoomed-in view of the experiment in Section~\ref{subsec:var_postgbit_networks}, where our servers were communicating for 10, respectively 5 seconds, then slept for 30 seconds. Note that at the beginning of each experiment, we made sure that the token-bucket budget is nearly empty. It is clear that during the first few seconds of the experiment the token-bucket budget gets completely deplenished. For each sending phase of 5 or 10 seconds, the system starts at a high QoS (10Gbps bandwidth), after a few seconds the budget is emptied, and subsequently the system assigns a low QoS (bandwidth of 1Gbps).
\begin{figure}
    \centering
    \includegraphics[width=0.94\columnwidth]{images/aws_emulation_validation.pdf}
    \vspace*{-0.4cm}
    \caption{Validation of the emulation of the token-bucket policy of the \amazon{}. The similar aspect of the two curves indicates that emulation is high-quality.}
    \label{fig:aws_emulation_validation}
    \vspace*{-0.4cm}
\end{figure}

==> gigabit_era.tex <==
\begin{table}[t]
\caption{Big data experiments on gigabit networks.}
\vspace*{-0.2cm}
\resizebox{0.98\columnwidth}{!}{
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Workload} & \textbf{Size} & \textbf{Network} & \textbf{Software} & \textbf{\#Nodes} \\ \midrule
HiBench           & Gigantic      & A-H, Figure~\ref{fig:bw_distribution}                                                          & \begin{tabular}[c]{@{}c@{}}Spark 2.4.0, \\ Hadoop 2.7.3\end{tabular}            & 16                  \\
TPC-DS            & SF-500        & A-H, Figure~\ref{fig:bw_distribution}                                                          & \begin{tabular}[c]{@{}c@{}}Spark 2.4.0,\\ Hadoop 2.7.3\end{tabular}             & 16                  \\ \bottomrule
\end{tabular}
}
\label{tab:exp_gigabit_era}
\vspace*{-0.5cm}
\end{table}

\section{Big Data in the \emph{Gigabit-Era}}\label{sec:gigabit_era}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{figure*}[!t]
    \centering
    \vspace*{-0.25cm}
    \includegraphics[width=0.92\textwidth]{images/tpcds_slowdown-1gbps-a-h.pdf}
    \vspace*{-0.65cm}
    \caption{TPC-DS slowdown variability presented as violin plots for running queries on bandwidth distributions A-H. The thickness of each violin represents the probability density, i.e., the likelihood of slowdown to be closer to a given value. For each query, the violin plot summarizes all the execution times across all A-H bandwidth distributions.}
    \label{fig:tpcsds_slowdown}
    \vspace*{-0.4cm}
\end{figure*}

% \begin{figure}[!t]
%     %\vspace*{-0.25cm}
%     \includegraphics[width=0.98\columnwidth]{images/hibench_slowdown-1gbps-a-h.pdf}
%     \vspace*{-0.5cm}
%     \caption{HiBench slowdown variability presented as violin plots when running queries on bandwidth distributions A-H. The thickness of each violin represents the probability density, i.e., the likelihood of slowdown to be closer to a given value. For each application, we summarized in the violin plot, all the execution times across all A-H bandwidth distributions. BS=Bayes, KM=Kmeans, PR=PageRank, S=Sort, TS=Terasort, WC=WordCount.}
%     \label{fig:hibench_slowdown}
%     \vspace*{-0.4cm}
% \end{figure}

% \begin{figure}[!t]
%     %\includegraphics[width=0.98\columnwidth]{images/ci-hibench.pdf}
%     \centering
%     \begin{subfigure}{\small{(a) Medians for HiBench-KM}}
%       \includegraphics[width=0.95\columnwidth]{images/ci-hibench.pdf}
%           \vspace{-0.2cm}
%       \label{fig:ci-hibench} 
%     \end{subfigure}
%     %\vspace{-0.22cm}
%     \begin{subfigure}{\small{(b) 0.9 quantiles for TPC-DS Q68}}
%       \includegraphics[width=0.95\columnwidth]{images/ci-tpcds.pdf}
%       \label{fig:ci-tpcds}
%     \end{subfigure}
%     \vspace{-0.5cm}
%     \caption{Medians and 0.9 quantile estimates, for HiBench-KM (a) and TPC-DS Q68 (b). All estimates are shown along with their 95\% confidence intervals (CIs) for performance measurements under the A-H network bandwidth distributions. We use $\diamond$ to depict estimates for each 50-run set. Judged by the most reliable 50-run CIs we consider, we show accurate estimates (inside those CIs) as \checkmark and inaccurate estimates (outside those CIs) as $\times$ for 3- and 10-run sets.}
%     \label{fig:poor_experimentation}
%     \vspace*{-0.3cm}
% \end{figure}

We characterize the behavior of big data workloads in clouds from gigabit-era variable networks. We uncover lessons learned and give recommendations for experiment design. Our main findings are:
\begin{description}[noitemsep,nosep,leftmargin=-0.03cm]
\item[F5.1] Network variability induces large amounts of variable application slowdown (up to 16X), for longer-running, batch-oriented applications (e.g., HiBench), and short running analytics queries (e.g., TPC-DS).
\item[F5.2] Experiments with a small number of repetitions result in highly volatile results, which can lead to unreliable conclusions; even experiments repeated 10 times frequently give inaccurate estimates of median performance. 
\item[F5.3] The effect of network variability on tail performance is even more pronounced than for median, meaning that good tail estimates require even more repetitions.
\end{description}

\iffalse
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.97\columnwidth]{images/SC_Emulation_Flow.png}
    \caption{Experimentation flow.}
    \label{fig:experiment_flow}
\end{figure}
\fi 

\textbf{Experiment Setup.} We perform the experiments described in Table~\ref{tab:exp_gigabit_era} on a 16-node cluster. Each node has 16 cores, 64GB memory, a 4TB HDD, and FDR InfiniBand network. Using the emulator presented in Section~\ref{sec:emulator}, we run the applications and queries in the HiBench~\cite{huang2010hibench} and TPC-DS~\cite{nambiar2006making} benchmark suites and subject them to the bandwidth distributions from Figure~\ref{fig:bw_distribution}. These are industrial-grade benchmarks, widely used in academia and industry; HiBench represents long-running, batch-processing workloads, while TPC-DS represents short-running analytics queries. Out of the TPC-DS suite, we select twenty queries, the same that are used in other big data performance studies~\cite{ousterhout2015making,erickson2014new}. We run each application or query repeatedly on each bandwidth distribution. Our experimentation flow is closely modeled after practice: the user submits an application via Spark~\cite{zaharia2012resilient} and the framework runs the workload in a distributed setup (i.e., a cluster). In our setup, the cluster emulates real-world cloud network variability.

\textbf{Variability Induced Slowdown.} We find that, even though networks are not a major bottleneck for big data applications (as discovered by Ousterhout et al.~\cite{ousterhout2015making}) network performance variability can still cause application slowdown, and the amount of that slowdown is highly variable. TPC-DS queries are significantly slowed down when running in gigabit-era performance-variable cloud networks. Moreover, due to the instability of the cloud, and many possible cloud bandwidth distributions, the slowdown itself is highly variable. Figure~\ref{fig:tpcsds_slowdown} shows the wide range of performance variability when running the TPC-DS queries on cloud bandwidth distributions A-H (Figure~\ref{fig:bw_distribution}). Figure~\ref{fig:hibench_slowdown} plots the result achieved when running the HiBench suite on all A-H bandwidth distributions. With only one exception, PageRank, all applications are heavily slowed down (i.e., 1.5-5X). Our results show that performance variability is not only manifesting within a single cloud, but also between clouds, leading to performance portability problems.

% \begin{figure}[!t]
%     %\includegraphics[width=0.98\columnwidth]{images/ci-hibench.pdf}
%     \centering
%     \begin{subfigure}{\small{(a) Medians for HiBench-KM}}
%       \includegraphics[width=0.95\columnwidth]{images/ci-hibench.pdf}
%           \vspace{-0.2cm}
%       \label{fig:ci-hibench} 
%     \end{subfigure}
%     %\vspace{-0.22cm}
%     \begin{subfigure}{\small{(b) 0.9 quantiles for TPC-DS Q68}}
%       \includegraphics[width=0.95\columnwidth]{images/ci-tpcds.pdf}
%       \label{fig:ci-tpcds}
%     \end{subfigure}
%     \vspace{-0.5cm}
%     \caption{Medians and 0.9 quantile estimates, for HiBench-KM (a) and TPC-DS Q68 (b). All estimates are shown along with their 95\% confidence intervals (CIs) for performance measurements under the A-H network bandwidth distributions. We use $\diamond$ to depict estimates for each 50-run set. Judged by the most reliable 50-run CIs we consider, we show accurate estimates (inside those CIs) as \checkmark and inaccurate estimates (outside those CIs) as $\times$ for 3- and 10-run sets.}
%     \label{fig:poor_experimentation}
%     \vspace*{-0.3cm}
% \end{figure}



\iffalse
\begin{figure*}
    \centering
    \includegraphics[width=\columnwidth]{images/hibench_slowdown.pdf}
    \caption{HiBench slowdown variability when running queries on bandwidth distributions A-H.}
    \label{fig:hibench_slowdown}
\end{figure*}
\fi

% \begin{figure*}[!t]
%     \centering
%     \vspace*{-0.25cm}
%     \includegraphics[width=0.98\textwidth]{images/tpcds_slowdown-1gbps-a-h.pdf}
%     \vspace*{-0.65cm}
%     \caption{TPC-DS slowdown variability presented as violin plots when running queries on bandwidth distributions A-H. The thickness of each violin represents the probability density, i.e., the likelihood of slowdown to be closer to a given value. For each application, we summarized in the violin plot, all the execution times across all A-H bandwidth distributions.}
%     \label{fig:tpcsds_slowdown}
%     \vspace*{-0.4cm}
% \end{figure*}

\begin{figure}[!t]
    %\vspace*{-0.25cm}
    \includegraphics[width=0.92\columnwidth]{images/hibench_slowdown-1gbps-a-h.pdf}
    \vspace*{-0.5cm}
    \caption{HiBench slowdown variability presented as violin plots. The thickness of each violin represents the probability density, i.e., the likelihood of slowdown to be closer to a given value. For each application, we summarized in the violin plot, all the execution times across all A-H bandwidth distributions. BS=Bayes, KM=Kmeans, PR=PageRank, S=Sort, TS=Terasort, WC=WordCount.}
    \label{fig:hibench_slowdown}
    \vspace*{-0.25cm}
\end{figure}

\begin{figure}[!t]
    %\includegraphics[width=0.98\columnwidth]{images/ci-hibench.pdf}
    \centering
    \begin{subfigure}{\small{(a) Medians for HiBench-KM}}
       \includegraphics[width=0.92\columnwidth]{images/ci-hibench.pdf}
           \vspace{-0.2cm}
       \label{fig:ci-hibench} 
    \end{subfigure}
    %\vspace{-0.22cm}
    \begin{subfigure}{\small{(b) 90th percentile for TPC-DS Q68}}
       \includegraphics[width=0.92\columnwidth]{images/ci-tpcds.pdf}
       \label{fig:ci-tpcds}
    \end{subfigure}
    \vspace*{-0.5cm}
    \caption{Medians and 90th percentile estimates, for HiBench-KM (a) and TPC-DS Q68 (b). Estimates are shown along with their 95\% confidence intervals (CIs) for performance measurements under the A-H network bandwidth distributions. We use $\diamond$ to depict estimates for each 50-run set. Judged by the most reliable 50-run CIs we consider, we show accurate estimates (inside those CIs) as \checkmark and inaccurate estimates (outside those CIs) as $\times$ for 3- and 10-run sets.}
    \label{fig:poor_experimentation}
    \vspace*{-0.4cm}
\end{figure}

\textbf{Sound Experimentation in the Gigabit Era.} Performed under variabile network conditions, experiment designs with few repetitions may lead to loose confidence intervals~(CIs), poor estimates, and erroneous conclusions. The effects of this can be seen in Figure~\ref{fig:poor_experimentation}, which plots estimates of 95\% nonparametric (asymmetric) CIs~\cite{Boudec2011Performance} for experiments on a range of different cloud bandwidth distributions (A--H from Figure~\ref{fig:bw_distribution}), with three different numbers of experiment repetitions (3\footnote{Three repetitions are insufficient to calculate CIs; we include medians for this experiment setup because it is representative of what is often found in the literature.}, 10, and 50). For these experiments, we find 50 repetitions to be enough to establish ``gold standards''---estimates with CI that are tight enough to be considered reliable. Then, we compare them to experiments with fewer repetitions (recall from Section~\ref{sec:litsurv} that many studies use 3, 5, or 10) to assess the quality of estimates in low-repetition experiments.

The top of Figure~\ref{fig:poor_experimentation} (part (a)) shows our estimates of \emph{medians} for the K-Means application from HiBench.
Our results show that experiments with three and ten repetitions offer poor estimates for the median: such ``early'' estimates fall outside of the trustworthy 
50-run CIs in  50\% of the studied cases. In other words, if we were to stop after three or ten repetitions, half of the time, we would report a performance value that is \emph{outside} the range that we would arrive at with a more sound experimental design.
It is also interesting to notice the behavior of network setup C, where three measurements attain a better estimate than ten measurements. This is clearly a result of chance and the evidence speaking for running larger numbers of experiment trials when evaluating systems that 
exibit even subtle performance variability. 
These CI-based insights complement the summary of estimation quality provided in Figure~\ref{fig:problem_statement}, and show how, in practice, running experiments with too few repetitions can result in inaccurate conclusions.

When analyzing big data systems the tail performance is an important measure~\cite{dean2013tail}.
It is even more difficult to get robust \emph{tail} performance estimates, as seen in the bottom half of Figure~\ref{fig:poor_experimentation}: here, only four of the 16 low-repetition experiments (and none of the three-repetition experiments) produce estimates that are within the bounds calculated from 50 repetitions. 
To obtain these results, 
we used TPC-DS measurements and the method from
Le~Boudec~\cite{Boudec2011Performance} to calculate nonparametric estimates for the 90th percentile performance, as well as their confidence bounds.
In contast with the medians, we notice that CIs for these tail estimates shrink for some cases and grow for others when we go from 10 to 50 measurements. 

Uncertainty grows as we learn more data about the distributions with higher variability.
Figure~\ref{fig:poor_experimentation}~(part (b)) demonstrates this effect (most visible for cloud~A) and depicts one of the cases with the least number of acceptable 3-run and 10-run estimates. 
The prinicipled way to address this uncertainty prescribes collecting measurements
until the CI is sufficiently tight (e.g., bounds are within 10\% of the estimate). Accordingly, the techniques described by Maricq et al.~\cite{maricq2018taming} can be adapted to consider $p$-quantiles and applied to larger sets of measurements obtained 
%on networks studied in this work.
using gigabit-era cloud networks.

%\tododmitry{Expand caption of Fig 14. Describe it and summarize the point that estimates obtained for small sets of of measurements can be quite inaccurate; also, in cloud C, we get lucky with 3 measurements and then unlucky with 10 -- it is important to consider that in practice.}


% \begin{figure}[!t]
%     %\vspace*{-0.25cm}
%     \includegraphics[width=0.98\columnwidth]{images/hibench_slowdown-1gbps-a-h.pdf}
%     \vspace*{-0.5cm}
%     \caption{HiBench slowdown variability presented as violin plots when running queries on bandwidth distributions A-H. The thickness of each violin represents the probability density, i.e., the likelihood of slowdown to be closer to a given value. For each application, we summarized in the violin plot, all the execution times across all A-H bandwidth distributions. BS=Bayes, KM=Kmeans, PR=PageRank, S=Sort, TS=Terasort, WC=WordCount.}
%     \label{fig:hibench_slowdown}
%     \vspace*{-0.4cm}
% \end{figure}

% \begin{figure}[!t]
%     %\includegraphics[width=0.98\columnwidth]{images/ci-hibench.pdf}
%     \centering
%     \begin{subfigure}{\small{(a) Medians for HiBench-KM}}
%       \includegraphics[width=0.95\columnwidth]{images/ci-hibench.pdf}
%           \vspace{-0.2cm}
%       \label{fig:ci-hibench} 
%     \end{subfigure}
%     %\vspace{-0.22cm}
%     \begin{subfigure}{\small{(b) 0.9 quantiles for TPC-DS Q68}}
%       \includegraphics[width=0.95\columnwidth]{images/ci-tpcds.pdf}
%       \label{fig:ci-tpcds}
%     \end{subfigure}
%     \vspace{-0.5cm}
%     \caption{Medians and 0.9 quantile estimates, for HiBench-KM (a) and TPC-DS Q68 (b). All estimates are shown along with their 95\% confidence intervals (CIs) for performance measurements under the A-H network bandwidth distributions. We use $\diamond$ to depict estimates for each 50-run set. Judged by the most reliable 50-run CIs we consider, we show accurate estimates (inside those CIs) as \checkmark and inaccurate estimates (outside those CIs) as $\times$ for 3- and 10-run sets.}
%     \label{fig:poor_experimentation}
%     \vspace*{-0.3cm}
% \end{figure}



==> post_gigabit_era.tex <==
https://www.overleaf.com/9421145846cwpnjzypvkfq
